Derivative-free stochastic bilevel optimization for inverse problems

Inverse problems are key issues in several scientific areas, including signal processing and medical imaging. Data-driven approaches for inverse problems aim for learning model and regularization parameters from observed data samples, and investigate their generalization properties when confronted with unseen data. This approach dictates a statistical approach to inverse problems, calling for stochastic optimization methods. In order to learn model and regularisation parameters simultaneously, we develop in this paper a stochastic bilevel optimization approach in which the lower level problem represents a variational reconstruction method formulated as a convex non-smooth optimization problem, depending on the observed sample. The upper level problem represents the learning task of the regularisation parameters. Combining the lower level and the upper level problem leads to a stochastic non-smooth and non-convex optimization problem, for which standard gradient-based methods are not straightforward to implement. Instead, we develop a unified and flexible methodology, building on a derivative-free approach, which allows us to solve the bilevel optimization problem only with samples of the objective function values. We perform a complete complexity analysis of this scheme. Numerical results on signal denoising and experimental design demonstrate the computational efficiency and the generalization properties of our method.

==> Intro.tex <==
%----------------------------------------------------------------------
%%% Intro
%----------------------------------------------------------------------
%!TEX root = ./ProxGrad_Main.tex
%

Bilevel optimization is a versatile tool for optimization problems in many applications arising in engineering, machine learning, inverse problems, among many others \cite{DempeAnnotated,Dempe:2002ve,BilevelLearningIEEE}. Most of these applications are massive in size and scalable optimization methods are in high demand. Such setting in particular arise in important applications such as meta-learning, hyper-parameter optimization \cite{pedregosa2016hyperparameter,franceschi2018bilevel}, adversarial networks \cite{Fiez:2020aa}, optimal experimental design \cite{Haber2008}, and reinforcement learning \cite{hong2023two}. Therefore, there has been increased interest in approaching bilevel optimization problem with the tools of first-order methods. In the case of deterministic data, the bilevel problem reads as 
\begin{equation}\label{eq:BL}
\min_{\by\in\scrY}\{\Psi(\by)\eqdef \min_{\bx\in\scrS(\by)} f(\bx,\by)\} \quad \text{where }\scrS(\by)\eqdef \argmin\{g(\bx,\by)\vert \bx\in\scrX\}.
 \end{equation}
A direct approach to this problem with gradient-based methods thus requires the estimation of $\nabla \Psi(\by)$, which is known in the literature as the \emph{implicit gradient} of the \emph{implicit function} $\Psi(\by)$. The vast majority of existing papers obtain this gradient information by the assumption that $\scrS(\by)$ is a singleton and $\scrX$ is a full domain (i.e. no implicit constraints). There is no straightforward way to extend these ideas to constrained lower level problems. The reason is that the arguments based on the implicit function theorem break down at the boundary of constrained domains, and therefore the implicit differentiation rules cannot be applied, even if a sufficient degree of smoothness is present in the problem data $f$ and $g$. However, even if classical tools from calculus are potentially applicable, there are good reasons to consider alternative approaches. To illustrate this statement, let us assume that we can apply the implicit function theorem to the implicit function $\Psi(\by)$. Computing the gradient formally leads then to the formula
\[
\nabla\Psi(\by)=\nabla_{y}f(\bx^{\ast}(\by),\by)-\nabla^{2}_{yx}g(\bx^{\ast}(\by),\by)\left[\nabla^{2}_{xx}g(\bx^{\ast}(\by),\by)\right]^{-1}\nabla_{x}f(\bx^{\ast}(\by),\by),
\]
with $\bx^{\ast}(\by)=\argmin_{\bx} g(\bx,by)$. 
We can see from this expression that direct applications of gradient methods to the implicit function actually requires to have an oracle that evaluates gradients and Hessians of the optimization problem's primitives at the lower level solutions. In the first-order black-box optimization setting, we do not have access to such information, which means that in a strict sense first-order methods cannot be applied. This observation is valid in deterministic as well as in stochastic setting, with the caveat that in stochastic formulation of \eqref{eq:BL} we actually must be explicit in which sense the lower level problem is solved for a given parameter $\by$. In this paper we are interested in solving a two-stage formulation of the stochastic bilevel optimization problem, reading as 
\begin{equation}\label{eq:SBL}
\begin{split}
 & \min_{\by\in\scrY}\{ \Ex_{\Pr_{0}}[F(\bx^{\ast}(\by,\xi_{2}),\xi_{1})]+r_{1}(\by)\} \\ 
\text{s.t.: } & \bx^{\ast}(\by,\xi_{2})\in\argmin_{\bx\in\scrX}\{g(\bx,\by,\xi_{2})+r_{2}(\bx)\} \quad\Pr_{0}-\text{a.e. }
\end{split}
\end{equation}
The stochastic setup embedding this optimization problem is given by a complete probability space $(\Omega_{0},\scrA_{0},\Pr_{0})$, carrying a random vector $\xi\eqdef(\xi_{1},\xi_{2})$ taking values in a product space $\Xi_{1}\times\Xi_{2}$. We do not assume any specific topological structure on these spaces. The interpretation of this model is as follows: The upper level objective is a population risk minimization problem where we aim to find optimal population parameters $\by\in\scrY$. The lower level problem solves a specific realization of a loss minimization problem, which depends on the population parameter $\by$ and the random noise term $\xi_{2}$. Hence, we seek in the lower level problem for a \emph{best-response} mapping, returning the optimal lower-level solution for given inputs $(\by,\xi_{2})$. Such an explicit hierarchical optimization problem is very common in applications, in particular in the statistical learning of inverse problems. 

\begin{example}[Bilevel learning in variational methods for inverse problems] 
\label{ex:population}
Let $(\xi_{1},\xi_{2})\in\Xi_{1}\times\Xi_{2}$ represent random elements defined on a probability space $(\Omega,\scrF,\Pr)$, representing the data of the problem. In inverse problems the task is to recover $x^{\dagger}\in\scrX$ from measured data $\xi_{2}\in\Xi_{2}$, where 
$$
\xi_{2}(\omega)=\bK(x^{\dagger})+Z(\omega)\qquad\forall \omega\in\Omega. 
$$
Here $\scrX\subseteq\Xi_{1}$ is the model parameter space and $\Xi_{2}$ is the data space. Moreover, $\bK:\scrX\to\Xi_{2}$ is a known continuous operator that maps model parameters to data, and $Z\in\Xi_{2}$ is a sample of a $\Xi_{2}$-valued random variable modeling observational noise. To learn the model parameters from observed measurements, variational methods have become the dominant paradigm \cite{DataInverse}. A data-driven approach for this task starts with an optimization formulation to recover model parameters from samples and regularization parameters. This leads to a paramterized optimization problem of the form 
$$
\bx^{\ast}(\by,\xi_{2})\in\argmin_{x\in\scrX}\{\scrL(\bK(\bx),\xi_{2})+\scrS_{\by}(\bx)\}\qquad\forall w\in\Xi_{2}\,
$$
where $\scrL:\Xi_{2}\times\Xi_{2}\to\R$ is a statistical loss function, typically related to a log-likelihood function of the data, and $\scrS_{\by}:\scrX\to\R\cup\{+\infty\}$ is a regularization function, incorporating a-prior information on the location of the model parameter, and preventing from overfitting. This regularization function is parameterized by a vector $\by\in\scrY$, which have to be provided before the recovery task. The parameter vector $\by$ are therefore treated as \emph{hyperparameters} of the model: Flexible parameters that can be calibrated. To assess the quality of the reconstruction parameter, bilevel learning searches for the optimal set of hyperparamters across the statistical population of data points. Hence, we are left with another optimization problem 
$$
\min_{\by\in\scrY}\{h(\by)+r_{1}(\by)\}, \quad h(\by)\eqdef \Ex_{\Pr}[F(\bx^{\ast}(\by,\xi_{2}),\xi_{1})]
$$
where $F:\scrX\times\Xi_{1}\to\R$ is a distance measure, which weights the discrepancy for every sample $(\xi_{1},\xi_{2})$ between the predicted model parameters $\bx^{\ast}(\by,\xi_{2})$ and the measurement $\xi_{1}$.  

%for inverse problems describe optimization based techniques extracting information on unknown parameters  A general formulation of this method starts with the definition of a reconstruction operator $\bx^{\ast}_{\by}:\Xi_{2}\to\scrX\equiv\Xi_{1}$, so that, for a given set of parameters $\by\in\scrY$, we make the prediction $\bx^{\ast}(\by,w)\equiv \bx^{\ast}_{\by}(w)$ on the image when the training input is $w\in\Xi_{2}$. The focus in this work is to learn selected features of the reconstruction operator from supervised learning. The population version of our learning problem thus reads as 
%\begin{align*}
%&\min_{\by}\Ex_{(\xi_{1},\xi_{2})\sim\mu}\left[F(\bx^{\ast}(\by,\xi_{2}),\xi_{1})\right]+r_{1}(\by)\,,\\ 
%&\bx^{\ast}(\by,w)\in\argmin_{x\in\scrX}\{D(\bK(\bx),w)+\rho_{\by}(\bx)+r_{2}(\bx)\}\qquad\forall w\in\Xi_{2}\,. 
%\end{align*}
%\swtd{For $\mu$-almost all $w\in\Xi_2$?} The solution of the upper level $\by^{\ast}$ corresponds to a Bayes estimator, though we do not assume that the %law $\mu$ is fully known. The upper level function $F(x,v):\scrX\times\scrX\to\R$ is a given statistical loss (e.g. $F(x,v)=\frac{1}{2}\norm{x-v}^{2}_{\scrX}$), and the function $\bx\mapsto D(\bK(\bx),w)$ is typically related to a log-likelihood function of the data. The mapping $\bK:\scrX\to\scrW$ is a forward operator, and the two mappings $r_{1}(\by),r_{2}(\bx)$ and $\rho_{\by}(\bx)$ are regularizers or penalty terms. 
\close
\end{example}

\begin{example}[Optimal experimental design]\label{ex:OED}
In optimal experimental design for inverse problems, the variable $\by$ captures design parameters for the measurement process. The inner problem models the inverse problem for given design parameters. Following similar notation as the previous example, this could be modeled as
\begin{align*}
    &\min_{\by}\Ex_{(\xi_{1},\xi_{2})\sim\mu}\left[F(\bx^{\ast}(\by,\xi_{2}),\xi_{1})\right]+r_{1}(\by)\,,\\ 
    &\bx^{\ast}(\by,w)\in\argmin_{x\in\scrX}\{D(\bK(\bx),\by, w)+r_{2}(\bx)\}\qquad\forall w\in\Xi_{2}\,,
    \end{align*}
where the design parameters may have a direct influence on the forward operator $\bK$. \swtd{$\scrW$ would also change in $\by$?}
\end{example}



\subsection*{Related Literature}
The literature on zeroth-order optimization methods is huge, and we can do no justice in summarizing the important literature. We only mention the most important references for our approach. 


\cite{Ghadimi:2013aa} is an early reference containing complexity results for unconstrained nonconvex stochastic optimization problems, assuming an exact stochastic gradient oracle is available to the optimizer. They establish an $O(n/\eps^{2})$ rate of achieving the accuracy $\Ex[\norm{\nabla f(x)}^{2}]\leq\eps$. 

\cite{Liu:2018aa} consider a variance reduced zeroth-order optimization method with variance reduction for finite-sum optimization problems. Relatedly, \cite{Rando:2022aa} refined the deterministic analysis in  \cite{Kozak:2022aa} to stochastic optimization using a zeroth-order gradient estimator using orthogonal directions. All these papers rely on the conventional assumptions in stochastic optimization (i.e. Lipschitz-smoothness, uniformly bounded variance). These assumptions are difficult to justify in bilevel optimization. 

In the context of hierarchical optimization, the recent paper \cite{Cui:2022aa} describes a zeroth-order stochastic approximation method based on increasing mini-batches. 

Bilevel optimization has gained immense popularity within the machine learning (ML) community. In particular, the stochastic bilevel case, as considered in this paper, described a highly relevant class of optimization models of ML. The state-of-the-art contributions are  

Bilevel optimization is by now a well-established toolbox in computational imaging and inverse problems. \cite{Ehrhardt:2021ab,Ehrhardt:2024aa} are recent references in this direction. 

The recent paper \cite{Pougkakiotis:2023aa} studies stochastic composite optimization problems in which the smooth part is expectation valued and weakly convex. They obtain complexity estimates in terms of the proximal gradient mapping of the smoothed problem. and claim that via this analysis they can derive an error bound on the distance to stationarity of the original problem. %Their analysis contains, unfortunately, a mistake, which seems crucial. 


%We complement and extend their analysis to the bilevel and stochastic setting, which is a much more general and challenging to deal with. In particular, we derive $\scrO(1/\sqrt{N})$ complexity guarantees, where Theorem 3.6 in \cite{Pougkakiotis:2023aa} obtain only guarantees optimality up to a plateau. 

In the convex case we provide complexity bounds for biased stochastic first-order methods, derived from Gaussian smoothing. Convergence and complexity results for biased stochastic gradient methods are rare in the literature. The closest result we could identify is \cite{AtcForMou17}. A recent survey for biased unconstrained SGD is \cite{Demi23}. Our results in the convex case extend the analysis of \cite{GhaLanHon16,Ghadimi:2013aa,Balasubramanian:2022aa} to the fully stochastic setting with biased gradient estimators. 


We emphasize that we consider the so-called two-point feedback setting. That is, given a random vector $\xi$, we assume that the stochastic composite function $F(\bx^{\ast}(\cdot,\xi_{2}),\xi_{1})$ can be evaluated at any point $y\in\scrY$ and another perturbed point $y+\eta u$.\swtd{Here, we are a bit less restrictive due to the allowed inexactness of the lower level} This assumption is needed in order to construct a finite difference estimator of the random gradient. Similar assumptions have been made in machine learning and computational statistics \cite{agarwal2010optimal,Duchi:2015aa,Ghadimi:2013aa}. The analysis of such more involved oracles is motivated by the sub-optimal oracle complexity of one-point feedback in stochastic zero-order optimization, measured either in terms of the approximation accuracy, or the dimension dependency. One-point feedback oracles can be traced back to \cite{NY83}.

A recent survey on bilevel optimization under uncertainty, with an emphasis on operations research, is \cite{Beck:2023aa}. 

\subsection*{Contributions and outline}
In this paper we analyze zeroth-order methods for bilevel problems of the form \eqref{eq:SBL}. The approach employs a smoothed stochastic gradient estimator to estimate the gradient of the upper level problem based on (inexact) evaluations of the lower level problem. 
We provide convergence guarantees and complexity bounds in terms of optimality for the smoothed upper level objective based on exact and inexact evaluations of the lower level problem. \swtd{It might be a matter of taste, but I would give more details in this section.  Moreover, I would emphasize the results of the inexact and convex analysis even more.} 

The outline of the paper is as follows. First, we introduce the mathematical setting and notation. We then formulate the stochastic bilevel problem, followed by the main results pertaining to smoothed stochastic gradient estimation and the resulting stochastic proximal gradient method. Then, numerical results are presented on relevant benchmark problems. Discussion and conclusions conclude the paper.

\section{Notation and preliminaries}
\tvl{we may want to harmonise the use of boldface, i.e., $\bx,\by$ vs. $x,y$.}
For a finite dimensional space $\scrE$, we denote by $\scrE^{\ast}$ its dual space. The value of a linear function $s\in\scrE^{\ast}$ at point $x\in\scrE$ is denoted by $\inner{s,x}$. We endow the spaces $\scrE$ and $\scrE^{\ast}$ with Euclidean norms 
\[
\norm{x}=\inner{Bx,x}^{1/2} \text{ and } \norm{s}_{\ast}=\inner{s,B^{-1}s}^{1/2},
\]
where $B=B^{\ast}$ represents the Riesz isomorphism, i.e. a positive definite linear operator from $\scrE$ to $\scrE^{\ast}$.  If $\Omega$ is a measurable space, we denote by $\scrB(\Omega)$ the Borel $\sigma$-algebra.  

In this paper we consider functions with different levels of smoothness. We say a function $h:\scrE\to\R$ belongs to class $\bC^{0,0}(\scrE)$ if there exists a constant $\lip_{0}(h)>0$ such that 
\[
|{h(x_{1})-h(x_{2})}|\leq \lip_{0}(h)\norm{x_{1}-x_{2}} \qquad\forall x_{1},x_{2}\in\scrE.
\]
We say $h\in\bC^{1,1}(\scrE)$ if 
\[
\norm{\nabla h(x_{1})-\nabla h(x_{2})}_{\ast}\leq \lip_{1}(h)\norm{x_{1}-x_{2}}.
\]
For a function $h\in\bC^{1,1}(\scrE)$ the following elementary descent estimate applies \cite[Lemma 1.2.3]{Nes18}
\begin{equation}\label{eq:descent}
h(x_{2})\leq h(x_{1})+\inner{\nabla h(x_{1}),x_{2}-x_{1}}+\frac{\lip_{1}(h)}{2}\norm{x_{2}-x_{1}}^2.
\end{equation}

For extended real-valued convex functions $h:\scrY\to[-\infty,\infty]$, we can define the convex subdifferential as the set-valued mapping $\partial h(\by)\eqdef \{g\in\scrY^{\ast}\vert h(\tilde{\by})\geq h(\by)+\inner{g,\tilde{\by}-\by}\quad\forall \tilde{\by}\in\scrY\}$. Elements of this set $g\in\partial h(\by)$ are called subgradients, and the inequality defining the set is called the subgradient inequality. A convex function is called proper if it never attains the value $-\infty$. \begin{definition}\label{def:deltaSubgradient}
Let $\delta\geq 0$. For a convex function $h:\scrY\to(-\infty,+\infty]$, we denote by $\partial_{\delta}h(\by)$ the set of dual vectors $g\in\scrY^{\ast}$ satisfying 
\begin{equation}
h(\tilde{\by})\geq h(\by)-\delta+\inner{g,\tilde{\by}-\by}\qquad \forall \tilde{\by}\in\scrY.
\end{equation}
The set $\partial_{\delta}h(\by)$ is the $\delta$-subdifferential of the convex function $h$. 
\end{definition}
Note that the above definition reduces naturally to the convex subdifferential by setting $\delta=0$. 

\begin{definition}
The proximal operator of a closed convex and proper function $g:\scrE\to(-\infty,\infty]$ is defined by  
\begin{equation}
\prox_{\alpha g}(\bx)\eqdef\argmin_{\bu\in\scrE}\{g(\bu)+\frac{1}{2\alpha}\norm{\bu-\bx}^{2}\}
\end{equation}
\end{definition}
The prox-operator is always 1-Lipschitz (non-expansive). Furthermore, we have the following well-known relations \cite{BauCom16}:
\begin{lemma}\label{lem:prox}
Let $(\scrE,\norm{\cdot})$ be a finite dimensional vector space and $f:\scrE\to(-\infty,\infty]$ a proper closed and convex  function. Then, for any $\bx,\bu\in\scrE$ the following are equivalent 
\begin{itemize}
\item $\bu=\prox_{f}(\bx)$ 
\item $\bx-\bu\in\partial f(\bu)$
\item $\inner{\bx-\bu,\by-\bu}\leq f(\by)-f(\bu)$ for any $\bx\in\scrE$.
\end{itemize}
\end{lemma}
We also make use of the Pythagorean identity on the Euclidean space $\scrY$ with inner product $\inner{B\cdot,\cdot}$:
\begin{equation}\label{eq:Pythagoras}
2\inner{\by-\bu,B(\bx-\by)} =\norm{\bx-\bu}^{2}-\norm{\bx-\by}^{2}-\norm{\by-\bu}^{2}
\end{equation}



We employ standard notation and concepts from probability theory (see e.g. \cite{YonZho99}). Let $(\Omega,\scrF,\Pr)$ be a probability space. A measurable function $f:(\Omega,\scrF,\Pr)\to\scrE$ is a random variable. The equivalence class of all measurable functions is denoted by $L^{0}(\Omega,\scrF,\Pr;\scrE)$. The law (distribution) of the random variable $f$ is the push-forward measure $\measP_{f}=\Pr\circ f^{-1}$ and constitutes a probability measure of $f(\Omega)\in\scrB(\scrE)$. The sub-sigma field of $f^{-1}(\scrF)$ of $\scrF$ is called the sigma-algebra generated by $f$, and denoted by $\sigma(f)$. Two elements $f,g\in L^{0}(\Omega,\scrF,\Pr;\scrE)$ are called independent if $\sigma(f)$ and $\sigma(g)$ are independent: For any two events $A\in\sigma(f)$ and $B\in\sigma(g)$, we have $\Pr(A\cap B)=\Pr(A)\Pr(B)$.  If $f:(\scrE,\scrB(\scrE))\to\R$ is a measurable function and $\xi\in L^{0}(\Omega,\scrF,\Pr;\scrE)$ then the mapping $f\circ\xi:(\Omega,\scrF)\to\R$ is $\sigma(\xi)$-measurable (Doob-Dynkin Lemma). We denote this composition as $f(\xi)(\omega)\eqdef f(\xi(\omega))\eqdef (f\circ\xi)(\omega)$, and often simply write $f(\xi)$ for this constructed random variable. In particular, we shall write $\Ex_{\Pr}[f(\xi)]=\int_{\Omega}f(\xi(\omega))\dif\Pr(\omega)$ for the integral of the measurable function $f(\xi):\Omega\to\R$. For $p\geq 1$, let $L^{p}(\Omega,\scrF,\Pr;\scrE)$ be the set of all random variables for which the integral 
\[
\Ex_{\Pr}\left[\abs{f}^{p}\right]\eqdef \int_{\Omega}\abs{f(\omega)}^{p}\dif\Pr(\omega)
\]
exists and is finite. This is a Banach space with norm $\abs{f}_{p}\eqdef \left(\Ex_{\Pr}\left[\abs{f}^{p}\right]\right)^{1/p}$. If $p=2$, then $L^{2}(\Omega,\scrF,\Pr;\scrE)$ is a Hilbert space with inner product
\[
\inner{f,g}_{L^{2}(\Omega,\scrF,\Pr;\scrE)}\eqdef \int_{\Omega}\inner{f(\omega),g(\omega)}\dif\Pr(\omega).
\]
Also, let $L^{\infty}(\Omega,\scrF,\Pr;\scrE)$ be the set of all essentially bounded $\scrF$-measurable random variables.

%In what follows, we often need bounds for the moments $M_{p}:=\int_{\scrE}\norm{u}^{p}\exp(-\frac{\norm{u}^{2}}{2})\dif u$. 
% \begin{lemma}[\cite{Nesterov:2017wm}, Lemma 1]
% \label{lem:Gaussbound}
% We have $M_{0}=1, M_{2}=n$ and for $p\in[0,2]$, 
% \begin{equation}\label{eq:Gaussboundlow}
% M_{p}\leq n^{p/2}. 
% \end{equation}
% If $p\geq 2$, then 
% \begin{equation}\label{eq:Gaussboundhigh}
% n^{p/2}\leq M_{p}\leq (p+n)^{p/2} 
% \end{equation}
% \end{lemma}
% \swtd{the last Lemma seems to be out of place, we may shift it to the discussion about Gaussian smoothing or into the appendix.} OK! 




==> OldComplexityAnalysis.tex <==
 \subsection{Complexity analysis}
 We start the analysis with a per-iteration bound on the evolution of the smoothed objective $\Psi_{\eta}$. 
 
\begin{lemma}\label{lem:AnalysisLem1}
Given $(\by,\bv)\in\scrY\times\scrY^{\ast}$ and $t>0$. Let $\by^{+}=P_{t}(\by,\bv)=\prox_{t r_{1}}(\by-t\bv)$. Then, for any $\tilde{\by}\in\scrY$, we have
 \begin{align*}
\Psi_{\eta}(\by^{+})&\leq\Psi_{\eta}(\tilde{\by})+\inner{\nabla h_{\eta}(\by)-\bv,\by^{+}-\tilde{\by}}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2t}\right)\norm{\by^{+}-\by}^{2}\\
&\left(\frac{\lip_{1}(h_{\eta})}{2}+\frac{1}{2t}\right)\norm{\tilde{\by}-\by}^{2}-\frac{1}{2t}\norm{\by^{+}-\tilde{\by}}^{2}.
\end{align*}
\end{lemma}
 \begin{proof}
 Let $\bp=\prox_{t r_{1}}(\bw)$. Lemma \ref{lem:prox}(iii) and eq. \eqref{eq:Pythagoras} in tandem yield 
 \begin{align*}
tr_{1}(\tilde{\by})-tr_{1}(\bp)&\geq\inner{B(\bw-\bp),\tilde{\by}-\bp}\\
&=\frac{1}{2}\norm{\bw-\bp}^{2}-\frac{1}{2}\norm{\bw-\tilde{\by}}^{2}+\frac{1}{2}\norm{\tilde{\by}-\bp}^{2}
\end{align*}
Call $\by^{+}=P_{t}(\by,\bv)$. Since $h_{\eta}\in\bC^{1,1}(\scrY)$, the descent lemma gives 
\[
h_{\eta}(\by^{+})\leq h_{\eta}(\by)+\inner{\nabla h_{\eta}(\by),\by^{+}-\by}+\frac{\lip_{1}(h_{\eta})}{2}\norm{\by^{+}-\by}^{2},
\]
and 
\[
h_{\eta}(\by)\leq h_{\eta}(\tilde{\by})+\inner{\nabla h_{\eta}(\by),\by-\tilde{\by}}+\frac{\lip_{1}(h_{\eta})}{2}\norm{\tilde{\by}-\by}^{2}
\]
Adding these two inequalities, we arrive at
\begin{equation}\label{eq:Lem1step1}
h_{\eta}(\by^{+})-h_{\eta}(\tilde{\by})\leq \inner{\nabla h_{\eta}(\by),\by^{+}-\tilde{\by}}+\frac{\lip_{1}(h_{\eta})}{2}\left(\norm{\by^{+}-\by}^{2}+\norm{\tilde{\by}-\by}^{2}\right)
\end{equation}
Setting $\bw=\by-tB^{-1}\bv$ so that $\bp=\by^{+}$, we see 
\begin{align*}
tr_{1}(\tilde{\by})-tr_{1}(\by^{+})&\geq \frac{1}{2}\norm{\by^{+}-(\by-tB^{-1}\bv)}^{2}-\frac{1}{2}\norm{\by-tB^{-1}\bv-\tilde{\by}}^{2}+\frac{1}{2}\norm{\tilde{\by}-\by^{+}}^{2}\\
&=\frac{1}{2}\norm{\by^{+}-\by}^{2}+t\inner{\bv,\by^{+}-\tilde{\by}}+\frac{1}{2}\norm{\by^{+}-\tilde{\by}}^{2}-\frac{1}{2}\norm{\tilde{\by}-\by}^{2}.
\end{align*}
Adding this to \eqref{eq:Lem1step1}, we conclude 
\begin{align*}
\Psi_{\eta}(\by^{+})&\leq\Psi_{\eta}(\tilde{\by})+\inner{\nabla h_{\eta}(\by)-\bv,\by^{+}-\tilde{\by}}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2t}\right)\norm{\by^{+}-\by}^{2}\\
&+\left(\frac{\lip_{1}(h_{\eta})}{2}+\frac{1}{2t}\right)\norm{\tilde{\by}-\by}^{2}-\frac{1}{2t}\norm{\by^{+}-\tilde{\by}}^{2}.
\end{align*}
 \end{proof}
 
Fix $k\in\{0,\ldots,K-1\}$ and call 
\begin{equation}
\bar{y}^{k}=T_{\eta,\alpha_{k}}(\by^{k})=P_{\alpha_{k}}(\by^{k},\nabla h_{\eta}(\by^{k})).
\end{equation}
Evaluating the estimate for the objective function in Lemma \ref{lem:AnalysisLem1} at the points $\by^{+}=\bar{\by}^{k},\by=\tilde{\by}=\by^{k},\bv=\nabla h_{\eta}(\by^{k})\in\scrY^{\ast}$, and the step size $t=\alpha_{k}$, we obtain 
\begin{align}
\Psi_{\eta}(\bar{\by}^{k})&\leq\Psi_{\eta}(\by^{k})+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}-\frac{1}{2\alpha_{k}}\norm{\bar{\by}^{k}-\by^{k}}^{2} \nonumber\\
&=\Psi_{\eta}(\by^{k})+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}.\label{eq:Psi1}
\end{align}
Repeating this evaluation, but now at the points $\tilde{\by}=\bar{\by}^{k},\by=\by^{k}$ and $\by^{+}=\by^{k+1}=P_{\alpha_{k}}(\by^{k},V_{k+1})$, we obtain the estimate
\begin{align*}
\Psi_{\eta}(\by^{k+1})&\leq\Psi_{\eta}(\bar{\by}^{k})+\inner{\nabla h_{\eta}(\by^{k})-V_{k+1},\by^{k+1}-\bar{\by}^{k}}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2\alpha_{k}}\right)\norm{\by^{k+1}-\by^{k}}^{2}\\
&+\left(\frac{\lip_{1}(h_{\eta})}{2}+\frac{1}{2\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}-\frac{1}{2\alpha_{k}}\norm{\by^{k+1}-\bar{\by}^{k}}^{2}.
\end{align*}
Using the Fenchel-Young inequality $\inner{\bv,\by}\leq \frac{1}{2}\left(\gamma\norm{\bv}^{2}_{\ast}+\frac{1}{\gamma}\norm{\by}^{2}\right)$ for $(\by,\bv)\in\scrY\times\scrY^{\ast}$ and $\gamma>0$, we can further bound the previous inequality by 
\begin{align*}
\Psi_{\eta}(\by^{k+1})&\leq\Psi_{\eta}(\bar{\by}^{k})+\frac{\alpha_{k}}{2}\norm{\nabla h_{\eta}(\by^{k})-V_{k+1}}^{2}_{\ast}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2\alpha_{k}}\right)\norm{\by^{k+1}-\by^{k}}^{2}\\
&+\left(\frac{\lip_{1}(h_{\eta})}{2}+\frac{1}{2\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}.
\end{align*}
Calling $\Delta W_{k+1}\eqdef V_{k+1}-\nabla h_{\eta}(\by^{k})$, and adding the above to the estimate \eqref{eq:Psi1}, we arrive at the fundamental recursion 
\begin{align*}
\Psi_{\eta}(\by^{k+1})&\leq\Psi_{\eta}(\by^{k})+\frac{\alpha_{k}}{2}\norm{\Delta W_{k+1}}^{2}_{\ast}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}\\
&+\left(\frac{\lip_{1}(h_{\eta})}{2}+\frac{1}{2\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2\alpha_{k}}\right)\norm{\by^{k+1}-\by^{k}}^{2}\\
&=\Psi_{\eta}(\by^{k})+\frac{\alpha_{k}}{2}\norm{\Delta W_{k+1}}^{2}_{\ast}+\left(\lip_{1}(h_{\eta})-\frac{1}{2\alpha_{k}}\right)\norm{\bar{\by}^{k}-\by^{k}}^{2}+\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2\alpha_{k}}\right)\norm{\by^{k+1}-\by^{k}}^{2}.
\end{align*}
Since $\bar{y}^{k}-\by^{k}=\alpha_{k}\scrG_{\eta,\alpha_{k}}(\by^{k})$ and $\by^{k+1}-\by^{k}=\alpha_{k}\tilde{\scrG}_{\eta,\alpha_{k}}(\by^{k})$, we can further bound the above expression by the following string of inequalities: Assume $\alpha_{k}\in(0,\frac{1}{\lip_{1}(h_{\eta})})$. Then, Lemma \ref{lem:RelationGradient} yields
\begin{align*}
\Psi_{\eta}(\by^{k+1})&\leq\Psi_{\eta}(\by^{k})+\frac{\alpha_{k}}{2}\norm{\Delta W_{k+1}}^{2}_{\ast}+\alpha^{2}_{k}\left(\lip_{1}(h_{\eta})-\frac{1}{2\alpha_{k}}\right)\norm{\scrG_{\eta,\alpha_{k}}(\by^{k})}^{2}\\
&+\alpha^{2}_{k}\left(\frac{\lip_{1}(h_{\eta})}{2}-\frac{1}{2\alpha_{k}}\right)\norm{\tilde{\scrG}_{\eta,\alpha_{k}}(\by^{k})}^{2}\\
&\leq \Psi_{\eta}(\by^{k})+\left(\alpha_{k}-\frac{\alpha^{2}_{k}\lip_{1}(h_{\eta})}{2}\right)\norm{\Delta W_{k+1}}^{2}_{\ast}+\left(\frac{3\lip_{1}(h_{\eta})\alpha^{2}_{k}}{4}-\frac{3\alpha_{k}}{4}\right)\norm{\scrG_{\eta,\alpha_{k}}(\by^{k})}^{2}.
\end{align*}
Rearranging the above, we continue with 
\begin{align*}
\frac{3\alpha_{k}}{4}(1-\alpha_{k}\lip_{1}(h_{\eta}))\norm{\scrG_{\eta,\alpha_{k}}(\by^{k})}^{2}\leq \Psi_{\eta}(\by^{k})-\Psi_{\eta}(\by^{k+1})+\frac{\alpha_{k}}{2}(2-\lip_{1}(h_{\eta})\alpha_{k})\norm{\Delta W_{k+1}}^{2}_{\ast}.
\end{align*}
Note that the cumulative process $\{(W_{k},\scrF_{k})\}_{k\geq 0}$, defined by $W_{0}\eqdef 0$ and $W_{k+1}\eqdef W_{k}+\Delta W_{k+1}$, is a square integrable martingale under the measure $\Pr$. Now, calling 
\[
\ca_{k}\eqdef \frac{3\alpha_{k}}{4}(1-\alpha_{k}\lip_{1}(h_{\eta}))\text{ and }\cb_{k}\eqdef \frac{\alpha_{k}}{2}(2-\lip_{1}(h_{\eta})), 
\]
and summing the above expression from $k=0$ to $k=K-1$, yields 
\begin{align*}
\Ex_{\Pr}\left[\sum_{k=0}^{K-1}\ca_{k}\norm{\scrG_{\eta,\alpha_{k}}(\by^{k})}^{2}\right]\leq \Psi_{\eta}(\by^{0})-\Psi^{\rm Opt}_{\eta}+\Ex_{\Pr}\left[\sum_{k=0}^{K-1}\cb_{k}\norm{\Delta W_{k+1}}^{2}_{\ast}\right],
\end{align*}
where $\Psi^{\rm Opt}_{\eta}\eqdef\inf_{\by\in\scrY}\Psi_{\eta}(\by)$. Since $\Delta W_{k+1}=V_{\eta,m_{k+1}}(\by^{k})$, we can invoke Lemma \ref{lem:errorbound}, to conclude that 
\begin{align*}
\Ex_{\Pr}\left[\sum_{k=0}^{K-1}\ca_{k}\norm{\scrG_{\eta,\alpha_{k}}(\by^{k})}^{2}\right]&\leq \Psi_{\eta}(\by^{0})-\Psi^{\rm Opt}_{\eta}+\sum_{k=0}^{K-1}\cb_{k}\frac{C_{n}}{m_{k+1}}\\
%&=\Psi(\by^{0})-\Psi^{\rm Opt}+[\Psi_{\eta}(\by^{0})-\Psi(\by^{0})]+[\Psi^{\rm Opt}-\Psi^{\rm Opt}_{\eta}]+\sum_{k=0}^{K-1}\cb_{k}\frac{C_{n}}{m_{k+1}}\\
%&\leq \Psi(\by^{0})-\Psi^{\rm Opt}+2\eta\lip_{0}(h)\sqrt{n}+\sum_{k=0}^{K-1}\cb_{k}\frac{C_{n}}{m_{k+1}}
\end{align*}
%where $C_{n}\eqdef (4+n)^{2}\left(\scrL_{0}(H)^{2}+\lip_{0}(h)^{2}\right)$. From here it follows that if $(1/m_{k+1})\in\ell^{1}_{+}(\N)$, and $\ca_{k}\geq\underline{\ca}>0$ for all $k\geq 0$, then, $\lim_{k\to\infty}\norm{\scrG_{\eta,\alpha_{k}}(\by^{k})}=0$ almost surely. To obtain rates, we need to specify the sample rate sequence $(m_{k})_{k\geq 1}$. 


==> WeakConvex.tex <==
%----------------------------------------------------------------------
%%% Weakly Convex
%----------------------------------------------------------------------
%!TEX root = ./ProxGrad_Main.tex
%

If it happens that the implicit function $h$ is weakly convex, we are in the framework studied in \cite{Pougkakiotis:2023aa}. In that case we show that a single-shot estimation strategy suffices to obtain convergence. We first work out a set of sufficient conditions that guarantee that the implicit function $\by\mapsto H(\by,\xi)$ is weakly convex. To simplify the notation, we treat in this section the random noise component as a parameter. To simplify the notation, we carry the parameter sometimes as a subscript with us, so that $F(\bx,\xi_{1})\equiv F_{\xi_{1}}(\bx)$ for $\xi_{1}\in\Xi_{1}$ fixed, and $\bx\in\scrX$ a variable input. 

\begin{definition}
A function $f:\scrX\to(-\infty,\infty]$ is said to be $\rho$-weakly convex if $x\mapsto f(x)+\frac{\rho}{2}\norm{x}^{2}_{\scrX}$ is convex.
\end{definition}
\begin{lemma}
Any $\rho$-weakly convex function $f:\scrX\to(-\infty,\infty]$ is locally Lipschitz continuous and directionally differentiable. 
\end{lemma}

\begin{lemma}
If $f\in\bC^{1,1}_{\lip_{1}(f)}(\scrX)$ then $f$ is $\rho=\lip_{1}(f)$-weakly convex. 
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}
$F_{\xi_{1}}:\scrX\to\R$ is a finite-valued and convex for any $\xi_{1}\in\Xi_{1}$. 
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By \cite[][Corollary 3.15]{Beck:2017aa}, the function $\bx\mapsto F_{\xi_{1}}(\bx)$ is subdifferentiable over $\scrX$. 
Together with assumption \ref{ass:UL}, we know that $\norm{z}_{\scrX^{\ast}}\leq\lip_{1}(F(\cdot,\xi_{1}))$ for all $z\in\partial F_{\xi_{1}}(\bx)$. To wit, recall the definition of the Fenchel conjugate $F^{\ast}_{\xi_{1}}:\scrX^{\ast}\to\bar{\R}$, defined as  
\begin{equation}
F^{\ast}_{\xi_{1}}(\bz)=\sup_{\bx\in\scrX}\{\inner{\bz,\bx}-F_{\xi_{1}}(\bx)\},
\end{equation}
Hence, for $\bx=\bar{\bx}_{\bz}$ a solution to this maximization problem, the Fermat principle informs us about the validity of the inclusion 
$$
0\in \bz+\partial F_{\xi_{{1}}}(\bar{\bx}_{\bz})\iff -\bz\in \partial F_{\xi_{{1}}}(\bar{\bx}_{\bz}).
$$
From this basic optimality condition, we immediately conclude that  $\norm{z}_{\scrX^{\ast}}\leq \lip_{1}(F(\cdot,\xi_{1}))$ for all $z\in\dom(F^{\ast}_{\xi_{1}})$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{ass:solutionmap}
The inner-level solution map $\bx^{\ast}(\cdot,\xi_{2})$ is $\lip_{1}(\bx^{\ast}(\cdot,\xi_{2}))$-Lipschitz smooth: For all $\bz\in\scrX^{\ast}$, we have 
\begin{equation}
\abs{\inner{\bz,\bx^{\ast}(\tilde{\by},\xi_{2})}-\inner{\bz,\bx^{\ast}(\by,\xi_{2})}-\inner{\bz,D_{y}\bx^{\ast}(\by,\xi_{2})}}\leq\frac{\lip_{1}(F(\cdot,\xi_{1}))\lip_{1}(\bx^{\ast}(\cdot,\xi_{2}))}{2}\norm{\tilde{\by}-\by}^{2}_{\ast}.
\end{equation}
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This assumption implies that for all $\bz\in\dom(F^{\ast}_{\xi_{1}})$ 
$$
\by\mapsto \inner{\bz,\bx^{\ast}(\by,\xi_{2})}+\frac{\lip_{1}(F(\cdot,\xi_{1}))\lip_{1}(\bx^{\ast}(\cdot,\xi_{2}))}{2}\norm{\by}^{2}_{\ast}
$$
is convex. Since $\bx\mapsto F(\bx,\xi_{1})\equiv F_{\xi_{1}}(\bx)$ is convex, we have the representation in terms of its Fenchel conjugate 
$
F_{\xi_{1}}(\bx)=\sup_{\bz\in\scrX^{\ast}}\{\inner{z,\bx}-F^{\ast}_{\xi_{1}}(\bz)\}$. It follows 
\begin{align*}
H(\by,\xi)&=F(\bx^{\ast}(y,\xi_{2}),\xi_{1})=\sup_{\bz\in\scrX^{\ast}}\{\inner{z,\bx^{\ast}(\by,\xi_{2})}-F^{\ast}_{\xi_{1}}(\bz)\}\\
&=\sup_{\bz\in\scrX^{\ast}}\{\inner{z,\bx^{\ast}(\by,\xi_{2})}+\frac{\lip_{1}(F(\cdot,\xi_{1}))\lip_{1}(\bx^{\ast}(\cdot,\xi_{2}))}{2}\norm{\by}^{2}_{\ast}-F^{\ast}_{\xi_{1}}(\bz)\}\\
&-\frac{\lip_{1}(F(\cdot,\xi_{1}))\lip_{1}(\bx^{\ast}(\cdot,\xi_{2}))}{2}\norm{\by}^{2}_{\ast}
\end{align*}
The first function is convex, being the pointwise supremum of convex functions. It follows that 
\[
H(\by,\xi)+\frac{\lip_{1}(F(\cdot,\xi_{1}))\lip_{1}(\bx^{\ast}(\cdot,\xi_{2}))}{2}\norm{\by}^{2}_{\ast}
\]
is convex, so that $H(\by,\xi)$ is weakly convex. 

==> smoothing_old.tex <==
%----------------------------------------------------------------------
%%%smoothing
%----------------------------------------------------------------------
%!TEX root = ./ProxGrad_Main.tex
%

We denote the unit ball in $\scrY$ by 
\[
\ball\eqdef\{\by\in\scrY\vert\norm{\by}_{\scrY}\leq 1\}=\{\by\in\scrY\vert\inner{B\by,\by}\leq 1\}.
\]
The unit sphere is denoted by $\sphere\eqdef\bd(\ball)\eqdef \{\by\in\scrY\vert\norm{\by}=1\}$. On the Euclidean space $\scrY$ we are given the Lebesgue measure $\dd\by$. 

The $n$-dimensional volume of the unit ball is $\Vol_{n}(\ball)=\frac{\pi^{n/2}}{\sqrt{\det(B)}\Gamma(\frac{n}{2}+1)}$, where $\Gamma(\cdot)$ is the Gamma function. Therefore, the measure 
$\dd\mu_{n}(\bf{u})\eqdef \1_{\{\bf{u}\in\ball_{n}\}}\frac{\dd\bf{u}}{\Vol_{n}(\ball_{n})}$ defines a uniform distribution on the unit ball in $\scrY$. Recall that $\Vol_{n-1}(\eps \sphere_{n})=\frac{n}{\eps}\Vol_{n}(\eps\ball_{n})$ for all $\eps>0$. 
\begin{definition}
Let $h:\in\C^{0,0}(\scrY)$. The spherical smoothing of $h$ is defined by
\begin{equation}\label{eq:smoothing}
h_{\eps}(\by)\eqdef \frac{1}{\Vol_{n}(\eps\ball_{n})} \int_{\eps \ball_{n}}h(\by+\bu)\dd \bu=\int_{\ball_{n}}h(\by+\eps\bw)\frac{\dd\bw}{\Vol_{n}(\ball_{n})}.
\end{equation}
\end{definition}
The following properties of the spherical smoothing can be deduced from \cite[Section 9.3.2]{NY83}; see also \cite[Lemma 1]{Cui:2022aa}. 
%%%%%%%%%%%%%%%%%%%
\begin{fact}
Let $h:\Rn\to\R$ be a continuous function that is $L_{h}$-Lipschitz continuous on $\scrX_{\delta}$. Then, for all $\bx,\by\in\scrX$, we have
\begin{align}
&\abs{h^{\delta}(\bx)-h^{\delta}(\by)}\leq L_{h}\norm{\bx-\by},\\
&\abs{h^{\delta}(\bx)-h(\bx)}\leq L_{h}\delta.
\end{align}
\end{fact}
%%%%%%%%%%%%%%%%%
Using Stoke's Theorem, one can easily show that 
\begin{equation}\label{eq:gradsmoothing}
\begin{split}
\nabla h^{\delta}(\bx)&=\frac{n}{\delta}\int_{\sphere_{n}}h(\bx+\delta \bv)\bv\frac{\dd\bv}{\Vol_{n-1}(\sphere_{n})}\\
&=\frac{n}{\delta}\Ex_{\bW\sim\Uniform(\sphere_{n})}[\bW h(\bx+\delta\bW)]\\
&=\frac{n}{\delta}\Ex_{\bW\sim\Uniform(\sphere_{n})}[\bW\left( h(\bx+\delta\bW)-h(\bx)\right)],
\end{split}
\end{equation}
where $\bW\sim\Uniform(\sphere_{n})$ means that $\bW$ is uniformly distributed on $\sphere_{n}$. A simple application of Jensen's inequality shows then that the spherical smoothing admits a Lipschitz continuous gradient, whose modulus depends on the smoothing parameter $\delta$. 
\begin{fact}
Let $h:\Rn\to\R$ be a continuous function that is $L_{h}$-Lipschitz continuous on $\scrX_{\delta}$. Then, for all $\bx,\by\in\scrX$, we have
\begin{equation}\label{eq:boundgradsmooth}
\norm{\nabla h^{\delta}(\bx)-\nabla h^{\delta}(\by)}\leq \frac{L_{h}n}{\delta}\norm{\bx-\by}.
\end{equation}
\end{fact}
The smoothed function and its gradient is used to construct a variance reduced gradient estimator for the implicit cost function of player $i$ in our hierarchical game problem. 

 Let $\phi:\scrY\to\R$ be a continuous function. Given a positive parameter $\eps>0$, we say 

\begin{equation}
\phi_{\eps}(\by)\eqdef \Int_{\ball(0,1)}\phi(\by+\eps\bu)
\end{equation}

where $\bu$ is a random vector in the unit ball $\ball$ in $\R^{d}$. Let $\partial\ball=\sphere$ denote the unit sphere in $\R^{d}$. Given a closed convex set $\scrX\subset\R^{d}$, we denote by $\setX^{\eta}\eqdef\scrX+\eta\ball.$. 

\begin{lemma}
Suppose $h:\R^{d}\to\R$ is continuous. The following holds true:
\begin{itemize}
\item $h_{\eta}$ is continuously differentiable over $\scrX$. In particular, 
\begin{equation}
\nabla_{x}h_{\eta}(x)=\frac{d}{\eta}\Ex_{v\in\eta\sphere}[h(x+v)\frac{v}{\norm{v}}].
\end{equation}
\item If $h\in C^{0,1}_{L_{h}}(\scrX^{\eta})$, then 
\begin{itemize}
\item $\abs{h_{\eta}(x)-h_{\eta}(y)}\leq L_{h}\norm{x-y}$,
\item $\abs{h_{\eta}(x)-h(x)}\leq L_{h}\eta$,
\item $\norm{\nabla_{x}h_{\eta}(x)-\nabla_{x}h_{\eta}(y)}\leq \frac{L_{h}d}{\eta}\norm{x-y}.$
\end{itemize} 
\item Define 
\[
